CACL: Community-Aware Heterogeneous Graph Contrastive Learning for Social Media Bot Detection

Social media bot detection is increasingly crucial with the rise of social media platforms. Existing methods predominantly construct social networks as graph and utilize graph neural networks (GNNs) for bot detection. However, most of these methods focus on how to improve the performance of GNNs while neglecting the community structure within social networks. Moreover, GNNs based methods still face problems such as poor model generalization due to the relatively small scale of the dataset and over-smoothness caused by information propagation mechanism. To address these problems, we propose a Community-Aware Heterogeneous Graph Contrastive Learning framework (CACL), which constructs social network as heterogeneous graph with multiple node types and edge types, and then utilizes community-aware module to dynamically mine both hard positive samples and hard negative samples for supervised graph contrastive learning with adaptive graph enhancement algorithms. Extensive experiments demonstrate that our framework addresses the previously mentioned challenges and outperforms competitive baselines on three social media bot benchmarks.

==> introduction.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figures/small figure.pdf}
    \caption{Illustration of considering diff-class nodes within one community as hard negative samples while same-class nodes between communities as hard positive samples. Based on these, graph contrastive learning is employed to push hard negative samples away and pull hard positive samples closer on the hypersphere.}
    \label{figure:small figure of idea}
\end{figure}

Social media bots, widely found within social networks, are software systems designed to interact with humans\cite{orabi2020bot_defination}, e.g., 9\% to 15\% active users on Twitter exhibit bot-like behaviors\cite{varol2017bot_exist}. Although social robots have brought convenience to people's daily life, including news broadcasts, online customer service, etc., their negative applications, such as online disinformation\cite{cresci2023bot_misinformation}, election interference\cite{cresci2020bot_election1,ferrara2017bot_election2}, extremism advocacy\cite{berger2015extreme_action}, seem to be more widespread and absolutely cannot be overlooked. To solve the above issues, numerous algorithms have been proposed to detect social media bots.

Existing works for social media bot detection primarily consist of feature based and graph based methods. In recent years, because feature engineering\cite{yang2020scalable_feature_engi,feng2021satar,dehghan2023node_structural} has proven to be incapable of addressing the challenge of generalization\cite{feng2022twibot-22}, graph convolutional neural networks\cite{kipf2016GCN} based models have been designed to leverage graph structure information. While homogeneous graphs\cite{ali2019detect_me_if_you_can_gcn} fail to model diverse relationships between social accounts, e.g., following, commenting, etc., heterogeneous graphs based methods, e.g., heterogeneous GCNs\cite{zhao2020heterogeneous_gcn}, relational GCNs\cite{feng2021botrgcn}, relational graph transformer\cite{feng2022RGT}, etc., can better capture semantic information from various relationships through aggregating both intra-relational and inter-relational information\cite{feng2022twibot-22}. Meanwhile, text graphs which consider texts from users as nodes are also constructed to consider the contextual consistency of users' texts\cite{lei2022BIC_text_graph}.

However, most of these efforts primarily focus on enhancing the performance of node features extraction by designing sophisticated convolutional networks, while neglecting the inherent graph structure information, i.e., social networks naturally divide into groups of nodes with denser connections inside each group and fewer connections between different groups\cite{liu2023botmoe,nguyen2014CommImportant,cherifi2019community_structure_in_graph}.\citep{newman2004newman_CommDense,tu2018user_same_interest} also show that members in one social community typically have some interests in common and tend to interact more frequently with each other than others their community.

The graph structure information mentioned above is important to understand the patterns of social  media\cite{comm_structure_important} and can be efficiently extracted by community-aware methods through partitioning vast social network into small-scale subgraphs\cite{rossetti2018graph_structure_by_comm}. Whereas, the crucial point is that both humans and bots are inevitably present in every community. For example, under a politically relevant tweet, it is often observed that responses from bots are intermingled with those from humans\cite{cresci2020bot_election1}. Due to the over-smoothing problem caused by graph convolution\cite{chen2020GCN_smooth}, GCNs based methods will result in highly similar feature representations of adjacent user nodes, and thus short distances in the feature space for diff-class nodes in one community, while far distances between same-class nodes in different communities\cite{zhou2020GCN_comm_smooth}. As illustrated in figure~\ref{figure:small figure of idea}, diff-class nodes in one community are defined as hard negative samples and same-class nodes in different communities are defined as hard positive samples. These hard samples pose a challenge for node classification.

To address the above challenge, we introduce supervised graph contrastive learning. By incorporating modified supervised contrastive loss, the GCNs based model is guided to focus on subtle differences between humans and bots within same community and push them away, while reasonably disregard distinct features among nodes of same class in different communities and pull them closer. In this manner, by continuously updating community structure and mining new hard samples, the representations of same-class nodes are consistently gathered on the hypersphere while those of diff-class are separated, which is beneficial to classification.

In this paper, we propose CACL(\textbf{C}ommunity-\textbf{A}ware Heterogeneous Graph \textbf{C}ontrastive \textbf{L}earning for Social Bot Detection), a graph contrastive learning framework capable of perceiving community structures. We employ community-aware module to perform community detection and mine both hard negative and positive samples at a coarse-grained level. We then utilize graph contrastive learning at a fine-grained level to deal with these hard samples. 
To generate contrastive graph, we introduce three adaptive data augmentation methods. Besides, by sharing the underlying feature extraction network, we align community-aware module and contrastive learning module to perform dynamically and adaptively hard samples mining. In summary, this paper makes the following contributions:
\begin{itemize}[leftmargin=*]
  \item We introduce community-aware module to dynamically extract community structures within social networks and perform both hard negative and positive samples mining.
  \item We propose a graph contrastive learning framework with community structure perception capabilities for the first time, and introduce three adaptive graph augmentation methods on both attribute-level and topology-level.
  \item We conduct comprehensive experiments on two social bot detection datasets to demonstrate the effectiveness and superiority of our CACL framework.
\end{itemize}

